Fast Execute-Only Memory for Embedded Systems

Remote code disclosure attacks threaten embedded systems as they allow attackers to steal intellectual property or to find reusable code for use in control-flow hijacking attacks. Execute-only memory (XOM) prevents remote code disclosures, but existing XOM solutions either require a memory management unit that is not available on ARM embedded systems or incur significant overhead. We present PicoXOM: a fast and novel XOM system for ARMv7-M and ARMv8-M devices which leverages ARM's Data Watchpoint and Tracing unit along with the processor's simplified memory protection hardware. On average, PicoXOM incurs 0.33% performance overhead and 5.89% code size overhead on two benchmark suites and five real-world applications.

==> tables/mem-beebs-summary.tex <==
%
% Code Size Overhead on BEEBS.
%
\begin{table}[pt]
\caption{Code Size Overhead on BEEBS}
\label{tbl:mem-beebs}
\centering
\sffamily
\footnotesize{
\resizebox{0.5\columnwidth}{!}{
\begin{tabular}{@{}lrr@{}}
\toprule
  & {\bf Baseline (KB)} & {\bf {\System} ($\times$)} \\
\midrule
  {\bf Min} & 29 & 1.0329 \\
  {\bf Max} & 41 & 1.0675 \\
  {\bf Geomean} & --- & 1.0614 \\
\bottomrule
\end{tabular}
}}
\end{table}

